Proceedings of the 19th International Overture Workshop

This volume contains the papers presented at the 19th International Overture Workshop, which was held in an hybrid format: online and physically at Aarhus, Denmark on 22th October 2021. This event was the latest in a series of workshops around the Vienna Development Method (VDM), the open-source project Overture, and related tools and formalisms. VDM is one of the longest established formal methods for systems development. A lively community of researchers and practitioners has grown up in academia and industry around the modelling languages (VDM-SL, VDM++, VDM-RT, CML) and tools (VDMTools, Overture, VDM VSCode extension, Crescendo, Symphony, the INTO-CPS chain, and ViennaTalk). Together, these provide a platform for work on modelling and analysis technology that includes static and dynamic analysis, test generation, execution support, and model checking. This workshop provided updates on the emerging technology of VDM/Overture, including collaboration infrastructure, collaborative modelling and co-simulation for Cyber-Physical Systems.

==> 1-Frasheri/Tables/experiments_table_cas2.tex <==
\begin{table}[]
\centering
\caption{Overview of experiments for Case-study 2}
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{\textbf{Case-study 1}} & \multicolumn{5}{c}{Parameters}                         \\

                                       & lA & mA & $t_s$ & $f_{data}$ & threaded     \\
                                       \midrule
Case 1                                 & 1         & 0.2s   & 0.1s      & every 0.1s & yes      \\
\midrule
Case 2                                 & 50         & 0.2s     & 0.1s       & every 0.1s & yes      \\
\midrule
Case 3                                 & 1         & 2s   & 0.1s      & every 0.1s & yes      \\
\midrule
Case 4                                 & 50         & 2s     & 0.1s       & every 0.1s & yes      \\
\midrule
Case 5                                 & 50         & 0.2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 6                                 & 200         & 2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 7                                 & 50         & 0.2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 8                                & 200         & 2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 9                                & 2         & 0.4s     & 0.1s       & every 0.2s & yes      \\
\midrule
Case 10                                & 5         & 0.4s     & 0.1s       & every 0.2s & yes      \\
\midrule
Case 11                                 & 2         & 2s     & 0.1s       & every 0.2s & yes      \\
\midrule
Case 12                                & 5         & 2s     & 0.1s       & every 0.2s & yes      \\



\bottomrule
\end{tabular}
\end{table}

==> 1-Frasheri/rbmqFMU_currentDesign.tex <==
\section*{RabbitMQ current design - Not part of the paper structure}
\begin{figure}
    \centering
    \resizebox{\textwidth}{!}{
    \input{Diagrams/rbmq-seq-diag_ENTERINITMODE}
    }
    \caption{Sequence Diagram for the function: $EnterInitializationMode$}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.9\textwidth}{!}{
    \input{Diagrams/rbmq-seq-diag_DOSTEP}
    }
    \caption{Sequence Diagram for the function: $DoStep$}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.9\textwidth}{!}{
    \input{Diagrams/rbmq-seq_CHECKSHD}
    }
    \caption{Sequence Diagram for the function: $checkSHD$, that deals with consumed system health data.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.6\textwidth}{!}{
    \input{Listings/msg2Send_SHD}
    }
    \caption{Message on system health data published by the rabbitMQFMU.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.6\textwidth}{!}{
    \input{Listings/msg2Consume_SHD}
    }
    \caption{Message on system health data consumed by the rabbitMQFMU}
    \label{fig:my_label}
\end{figure}

==> 3-Oda/acronyms.tex <==
\newacronym{ast}{AST}{Abstract Syntax Tree}
\newacronym{ct}{CT}{Combinatorial Testing}
\newacronym{czt}{CZT}{Community Z Tools}
\newacronym{dap}{DAP}{Debug Adapter Protocol}
\newacronym{dbgp}{DBGP}{Common DeBugGer Protocol}
\newacronym{gui}{GUI}{Graphical User Interface}
\newacronym{ide}{IDE}{Integrated Development Environment}
\newacronym{lsp}{LSP}{Language Server Protocol}
\newacronym{poc}{PoC}{Proof of Concept}
\newacronym{pog}{POG}{Proof Obligation Generation}
\newacronym{slsp}{SLSP}{Specification Language Server Protocol}
\newacronym{vdm}{VDM}{Vienna Development Method}
\newacronym{vscode}{VS Code}{Visual Studio Code}


==> 3-Oda/listings/LoC_v1.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|}
\hline
\textbf{Directory/File} & \textbf{Code}                     & \textbf{Comment}                 & \textbf{Blank}                   & \textbf{Total}                    \\ \hline
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                                                                                                        \\ \hline
dap                     & 699                               & 450                              & 186                              & 1335                              \\ \hline
json                    & 551                               & 184                              & 128                              & 863                               \\ \hline
lsp                     & 1242                              & 492                              & 257                              & 1991                              \\ \hline
rpc                     & 177                               & 137                              & 54                               & 368                               \\ \hline
vdmj                    & 1940                              & 429                              & 374                              & 2743                              \\ \hline
workspace               & 1438                              & 123                              & 251                              & 1812                              \\ \hline
\textbf{Sum}            & \textbf{6047}                     & \textbf{1815}                    & \textbf{1250}                    & \textbf{9112}                     \\ \hline
\multicolumn{5}{|c|}{VS Code Extension}                                                                                                                               \\ \hline
extension.ts            & \multicolumn{1}{l|}{150}          & \multicolumn{1}{l|}{30}          & \multicolumn{1}{l|}{34}          & \multicolumn{1}{l|}{214}          \\ \hline
package.json            & \multicolumn{1}{l|}{131}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{132}          \\ \hline
syntax highlight        & \multicolumn{1}{l|}{374}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{374}          \\ \hline
\textbf{Sum}            & \multicolumn{1}{l|}{\textbf{655}} & \multicolumn{1}{l|}{\textbf{30}} & \multicolumn{1}{l|}{\textbf{35}} & \multicolumn{1}{l|}{\textbf{720}} \\ \hline
\end{tabular}
\end{table}

==> 3-Oda/listings/LoC_v2.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|llllll}
\cline{1-5} \cline{7-11}
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                               & \multicolumn{1}{l|}{} & \multicolumn{5}{c|}{VS Code Extension}                                                                                                                                                                \\ \cline{1-5} \cline{7-11} 
\textbf{Directory/File} & \textbf{Code} & \textbf{Comment} & \textbf{Blank} & \textbf{Total} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Directory/File}} & \multicolumn{1}{r|}{\textbf{Code}} & \multicolumn{1}{r|}{\textbf{Comment}} & \multicolumn{1}{r|}{\textbf{Blank}} & \multicolumn{1}{r|}{\textbf{Total}} \\ \cline{1-5} \cline{7-11} 
dap                     & 699           & 450              & 186            & 1335           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{extension.ts}            & \multicolumn{1}{l|}{150}           & \multicolumn{1}{l|}{30}               & \multicolumn{1}{l|}{34}             & \multicolumn{1}{l|}{214}            \\ \cline{1-5} \cline{7-11} 
json                    & 551           & 184              & 128            & 863            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{package.json}            & \multicolumn{1}{l|}{131}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{1}              & \multicolumn{1}{l|}{132}            \\ \cline{1-5} \cline{7-11} 
lsp                     & 1242          & 492              & 257            & 1991           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{syntax highlight}        & \multicolumn{1}{l|}{374}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{0}              & \multicolumn{1}{l|}{374}            \\ \cline{1-5} \cline{7-11} 
rpc                     & 177           & 137              & 54             & 368            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Sum}}            & \multicolumn{1}{l|}{\textbf{655}}  & \multicolumn{1}{l|}{\textbf{30}}      & \multicolumn{1}{l|}{\textbf{35}}    & \multicolumn{1}{l|}{\textbf{720}}   \\ \cline{1-5} \cline{7-11} 
vdmj                    & 1940          & 429              & 374            & 2743           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
workspace               & 1438          & 123              & 251            & 1812           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\textbf{Sum}            & \textbf{6047} & \textbf{1815}    & \textbf{1250}  & \textbf{9112}  &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\end{tabular}
\end{table}

==> 3-Oda/sections/evaluation.tex <==
In this section we discuss the implementation effort carried out in order to support the \gls{lsp}, \gls{slsp} and \gls{dap} protocols for VDMJ and the efforts needed on the client side to provide \gls{vdm} support.
This is compared to the efforts necessary to migrate the Overture language features to a different \gls{ide} without using the protocols as performed in \cite{Tran&19}.
Finally, we discuss to which extent it is currently possible to decouple specification language features from development tools using standardised protocols and what is required to have fully decoupled language support using protocols.


\subsection{Assessing the Implementation Effort}
% Page budget: 1
% \\Writer: J+F (+ Maybe Nick)
% \begin{itemize}
%     \item Was it straight forward to implement the extension? (Lines of code)
%     \item Was it straight forward to implement protocols in the server? (Lines of code)
% \end{itemize}
% \todo{Maybe relate to the paper: Tran19}
% \todo{Don't know if the comparison is still too thin..?}

The implementation effort is quantified by counting the Lines of Code (LoC) used for implementing support for a given protocol and the features it enables.
Providing support the protocols for VDMJ requires 7855 LoC, whereas support for \gls{vdm} in the \gls{vscode} extension only requires 1880 LoC where most are used for the new \gls{slsp} features.
The few lines of code for the extension can mainly be attributed to the generic \gls{lsp} and \gls{dap} protocol implementations exposed by the \gls{vscode} API\footnote{See \url{https://code.visualstudio.com/api/references/vscode-api}}.

A detailed overview of the lines needed to implement the language support is shown in \Cref{tab:LoCOverview}. 
In the table the `json' and `rpc' directory contain a basic JSON/RPC system; `dap' and `lsp' are the protocol handlers for each; `lsp/lspx' is the handler for SLSP; `vdmj' is the DebugLink and visitors to implement the various features (i.e.\ these link to the VDMJ jar); and `workspace' contains the code to maintain the collection of files. 
For the \gls{vscode} extension `LSP client' and `DAP client' is the setup of each client; `POG' and `CT' is the protocol handlers and GUI support for each feature; `syntax highlighting' contains the TextMate grammars for \gls{vdm}; and `SLSP Protocol' is the definition of the \gls{slsp} protocol and expansion of the LSP client.

\input{tables/LoCOverview}

% It should also be noted that the LoC for the server implementation includes an implementation of the JSON-RPC base protocol used for messages specified in the \gls{lsp} protocol.
% This could have been replaced with existing packages such as LSP4J\footnote{See \url{https://github.com/eclipse/lsp4j}} which could reduce the workload and LoC.
% However, LSP4J and all its dependencies amounts to about 4Mb, whereas the jar containing all the \gls{lsp} and \gls{dap} protocol support for VDMJ has a size about 130Kb.
% Thus, even though using LSP4J may save some time it comes at the cost of a considerable memory increase.

A comparison between LoC for the \gls{vscode} extension, migrating Overture to Emacs (as in \cite{Tran&19}) and the Overture IDE (version 3.0.1) not counting the core is seen in \Cref{tab:LoCCompare}. 
From the comparison we find that the \gls{vscode} extension requires more code than the Emacs migration but Overture consists of far more LoC than both.
However, if we only look at the \gls{lsp} and \gls{dap} client support that covers all the normal programming language features they only require 210 LoC.
The \gls{slsp} parts of the extension are made almost generic, hence these parts can be reused for other specification languages to enable support for the same features in \gls{vscode}.

For VDMJ to support the protocols it requires considerably more LoC compared to the Emacs approach from \cite{Tran&19}, which weights against the protocol approach for enabling \gls{vdm} feature support.
However, the protocol solution is a standardisation of the decoupling, hence the server supporting the language features (in this case VDMJ) only has to be implemented once to be used with any development tool supporting the protocols. 
In comparison, the \gls{vscode} extension and migration of the Overture language core to another development tool, as done with Emacs, must be performed for each \gls{ide} that is to be supported.
Furthermore, the Overture migration depends on Emacs packages, which may not exist in other \glspl{ide} or have a different interface.
Thus, the analysis of finding suitable packages for another \gls{ide} will have to be repeated, possibly making the server solution faster to implement in a new \gls{ide}.

\input{tables/LoCCompare}

To provide a fair comparison between the three implementation efforts, we compare the features that are available in each.
The comparison is done by the same set of features as in \cite{Tran&19}, this is found in \Cref{tab:featureCompare}.
As illustrated, the Overture IDE and the Emacs migration both support more features than the \gls{vscode} extension.
However, some of the features provided by the Emacs migration is only available through a command-line interface and not by a \gls{gui}.
\gls{vscode} does support implementation of integrated command-line interfaces like the Emacs migration, however the implementation efforts related to this are unknown.
Providing this kind of command-line interface has intentionally been left out of the \gls{vscode} extension, as we wanted to replicate the workflow from Overture.

\input{tables/featureCompare}


\subsection{Protocol Coverage of Language Features}
\label{sec:ProtocolCoverage}
% Page budget: 1.5
% \\Writer: J
% \begin{itemize}
%     \item Introduction to full set of features needed to replace Overture. (+ Overview picture like the one in the thesis)
%     \item Which features are covered by DAP?
%     \item Which features are covered by LSP?
% \end{itemize}

% The current extension is mainly focused on using the standard protocols \gls{lsp} and \gls{dap} to support \gls{vdm}. 
% However, as these protocols are developed with programming languages in mind, many features for supporting specification languages, such as those found for \gls{vdm} in Overture, are not supported by these protocols.
To get an overview of the specification language features that are covered by the protocols, we have examined and grouped the features that are sought after to support specification languages such as \gls{vdm}, B and Z.
This is illustrated in \Cref{fig:ProtocolCoverage}, where the language features have been divided into four categories:
\begin{enumerate}
    \item \textbf{Editor}: features that support writing a given specification, e.g.\ type- and syntax-checking.
    \item \textbf{Translation}: features that support translating a specification to other formats, e.g.\ executable code and LaTeX.
    \item \textbf{Validation}: features that support validation of a specification.
    \item \textbf{Verification}: features that support verification of a specification.
\end{enumerate}

\begin{figure}[htbp]
    \centering
        \includegraphics[width=0.53\textwidth]{figures/SLSP_Protocol_coverage.pdf}
    \caption{Specification language features covered by existing protocols}
    \label{fig:ProtocolCoverage}
\end{figure}

% The proof-of-concept implementation is able to provide the features syntax checking, type checking and go-to functionality.
As a result of the initial implementation and by comparing the features supported by the \gls{lsp} protocol with the features from Overture, it is found that the protocol is able to support all of the editor related features except syntax highlighting.
Thus, specification languages that benefits from the editor features found in \Cref{fig:ProtocolCoverage}, can use a direct implementation of the \gls{lsp} protocol to support this feature set.

% The extension is also able to provide syntax highlighting, however this handled on the client side and therefore it is not using the \gls{lsp} protocol.

The \gls{dap} protocol can be used for decoupling the debugging feature as it supports common debug functionality such as different types of breakpoints, variable values and more.
This is useful for specification languages that allow execution of specifications.

Additionally, the \gls{slsp} extension to \gls{lsp} facilitates support for both \gls{pog} and \gls{ct}. 
As found in \Cref{fig:ProtocolCoverage} there are still many features related to specification languages that are not supported by protocols.
Thus, in order to achieve fully decoupled language server support for \gls{vdm} one or more protocols must be developed that support the remaining features.
From our development of \gls{slsp} we believe that it is possible to develop a language-agnostic protocol to support all of these features, which should make it possible to apply the protocol to multiple specification languages and potentially increase the industrial uptake of specification languages.


==> 3-Oda/sections/implementation.tex <==
% \todo{We should probably publish the extension to the marketplace such that readers can better understand what is talked about}
% \todo{How are we on code snippets? go or no-go? What should they provide if included?}


The support for \gls{vdm} in \gls{vscode} is accomplished using an extension that communicates with a language server based on the language support found in VDMJ, as illustrated in \Cref{fig:ExtensionArchitecture}.
The standard protocols \gls{lsp} and \gls{dap} are developed with programming languages in mind. 
This means that the specification language features that are common for these languages are not supported, \eg \gls{pog} and \gls{ct}, as discussed in \Cref{sec:ProtocolCoverage}.
To compensate for this we have developed the \gls{slsp} protocol, which is introduced in the section \Cref{sec:slspIntroduction}. 
Followed by a description of the components that the \gls{vscode} extensions\footnote{The extensions can be found at: \url{https://github.com/jonaskrask/vdm-vscode}} are comprised of and how they have been implemented.
Finally, we describe the work put into VDMJ to provide support for the protocols.

\begin{figure}[htb]
    \centering
        \includegraphics[width=1\textwidth]{figures/ExtensionArchitecture_v3.pdf}
    \caption{Overview for the suggested extension architecture}
    \label{fig:ExtensionArchitecture}
\end{figure}

\subsection{Specification Language Server Protocol}
\label{sec:slspIntroduction}
The purpose of the \gls{slsp} protocol is to facilitate support for specification language specific features using the same architecture as for \gls{lsp} and \gls{dap}.
The \gls{slsp} protocol is an extension to the \gls{lsp} protocol.
This means that it uses the same base protocol as \gls{lsp} and relies on functionality from \gls{lsp} such as the synchronisation between client and server.
The protocol is developed with the intention that it should also be usable by other languages than \gls{vdm} and possibly be included in the \gls{lsp} specification. 
Hence, the \gls{slsp} protocol uses language neutral data types, which allows the client to be language-agnostic enabling it to be used with any server that supports the \gls{slsp} protocol.
At the time of writing the \gls{slsp} protocol defines messages to support \gls{pog} and \gls{ct}, and it is used in the \gls{vscode} extension for those features. 

\subsection{Visual Studio Code Extension}
% Page budget: 3
% \\Writer: J
% \begin{itemize}
%     \item Overall description of extension concept (also has extension generator)
%     \item What components does it include
%     \item Activation. (Language trigger. Starting server)
%     \item The workspace concept.
% \end{itemize}
\Gls{vscode} operates with a rich extensibility model that enables users to include support for different programming languages, debuggers and various tools to support the development workflow, by downloading extensions from the \gls{vscode} extensions marketplace\footnote{See \url{https://marketplace.visualstudio.com/vscode}}.
This also enables developers to make extensions that they find missing from the marketplace, which is how \gls{vdm} is supported in \gls{vscode}; by creating an extension for each \gls{vdm} dialect.
The extensions include a \gls{slsp} client and a \gls{dap} client.
Besides communicating with the server the extension also has the responsibility of doing syntax highlighting as this is not supported in any of the protocols.

As illustrated in \Cref{fig:ExtensionArchitecture}, \gls{vscode} includes generic support for both the \gls{lsp} and \gls{dap} protocols which allows the client implementation to be carried out with little effort.
The generic protocol support provides the extension with handlers for all the \gls{lsp} and \gls{dap} messages which include code to synchronise the editor and the server, handling of the editor navigation and displaying messages from the server.
Thus, the extension provides configuration of the generic protocol support, launching and connecting to the server, syntax highlighting, and the \gls{gui} to support the \gls{slsp} features.
\Cref{fig:VSCodeSnippet_pog} depicts the \gls{vscode} environment with the VDM-SL extension active.


\begin{figure}[htb]
    \centering
        \includegraphics[width=1\textwidth]{figures/VSCodeSnippet_pog.pdf}
    \caption{VDM-SL VS Code Extension: (1) Main Editor; (2) Project Explorer; (3) File Outline; (4) Proof Obligation View}
    \label{fig:VSCodeSnippet_pog}
\end{figure}

\subsubsection{Syntax Highlighting:}
% \begin{itemize}
%     \item Supported in the extension.
%     \item TextMate grammar and Oniguruma regular expressions.
% \end{itemize}
Syntax highlighting in \gls{vscode} is handled on the client side as it is not supported by the protocols. 
Instead syntax highlighting is performed using TextMate grammars \cite{Gray07}. 
The TextMate grammars are structured collections of Oniguruma regular expressions\footnote{See \url{https://github.com/kkos/oniguruma}}, implemented using a JSON schema. 
The grammar file specifies a set of rules, that is used with pattern matching to transform the visible text into a list of tokens and colour these according to a colour scheme.

\subsubsection{Specification Language Server Protocol Client:}
% \begin{itemize}
%     \item Client implementation (A few lines of code..)
% \end{itemize}
As custom for language extensions the VDM extensions are activated when a file with a matching file format is opened, \eg opening a `\texttt{.vdmsl}' file actives the VDM-SL extension.
On activation the client launches the server and connects to it.
When connected, the client forwards all relevant information to the server using the \gls{lsp} protocol. 
Furthermore, any responses or notifications from the server triggers feedback to the user, which is handled by the generic \gls{lsp} client integration in \gls{vscode}.
In addition to setting up the support for \gls{lsp} the client also provides customised \gls{gui} views to support \gls{pog} and \gls{ct}. This is not directly supported by \gls{vscode} and \gls{lsp} since these features are not commonly used for traditional programming languages. 

%\todo{More juice on POG and CT?}
The \gls{pog} view, illustrated in \Cref{fig:VSCodeSnippet_pog}, provides a list of the proof obligations for a specification, where expanding an element displays the actual proof obligation.
The view is implemented using the \gls{vscode} Webview API\footnote{See \url{https://code.visualstudio.com/api/extension-guides/webview}.}, which is customised using CSS, HTML and JavaScript.

The \gls{ct} view, illustrated in \Cref{fig:VSCodeSnippet_ct}, shows the tests that are generated based on the traces in the specification, these are structured in a tree view.
Traces can be fully or partially executed using either an execution filter or executing a test group at a time. 
A tests execution sequence and result is displayed in a separate tree view.
Tests can also be debugged, which is facilitated using the \gls{dap} protocol.
The \gls{ct} view is implemented using the \gls{vscode} Tree View API\footnote{See \url{https://code.visualstudio.com/api/extension-guides/tree-view}.}. which reduces the complexity of implementing a view.

\begin{figure}[htb]
    \centering
        \includegraphics[width=1\textwidth]{figures/VSCodeSnippet_ct.pdf}
    \caption{VDM-SL VS Code Extension: (1) Combinatorial Testing View; (2) Test Result View; (3) Debug Console}
    \label{fig:VSCodeSnippet_ct}
\end{figure}


\subsubsection{Debug Adapter Protocol Client:}
% \begin{itemize}
%     \item Client implementation.
%     \item How is it activated.
% \end{itemize}
The \gls{dap} protocol support is added to the client by specifying a \texttt{DebugAdapterDescriptorFactory} which establishes the connection between the generic debugger client and the server upon starting a debug session.
This would normally include launching a \gls{dap} server and connect to it.
However, as the \gls{lsp} and \gls{dap} server is combined into one we simply connect to the port specified for \gls{dap} communication. 
% An illustration of the debugger interface in \gls{vscode} is seen in \Cref{fig:VSCodeSnippet_debug}.

% \begin{figure}[htb]
%     \centering
%         \includegraphics[width=1\textwidth]{figures/VSCodeSnippet_debug.pdf}
%     \caption{VDM-SL VS Code Extension: (1) Main Editor; (2) Debug Console; (3) Proof Obligation View; (4) Combinatorial Testing View; (5) Test Result View}
%     \label{fig:VSCodeSnippet_debug}
% \end{figure}


\subsection{Enabling the use of LSP and DAP in VDMJ}
% Page budget: 3
% \\Writer: Nick

% \subsubsection{LSP Support}
% \begin{itemize}
%     \item What has been done to conform to the protocol.
%     \item Supporting the messages (lsp4j? )
%     \item Workspace/project handling (Using LSP workspace features?)
    
% \end{itemize}

% \subsubsection{DAP Support}
% \begin{itemize}
%     \item What did it require to make the Debug Adapter
% \end{itemize}

Internally, VDMJ provides a set of language services to enable VDM specifications to be processed, and by default the coordination of these services is handled by a command-line processor. So for example, a Parser service is used to analyse a set of VDM source files to produce an Abstract Syntax Tree (AST); if there are no syntax errors, that AST is further processed by a Type Checker; and if there are no type errors, the tree is further processed by an Interpreter (in a read-eval loop) or by a Proof Obligation Generator. If the Interpreter encounters a runtime problem or a debug breakpoint, it stops and interacts with the command-line to allow the user to examine the stack and variables, for example.

Although the command-line is the default way to interact with VDMJ, this is not assumed in the design. An alternative means to interact is provided using the DBGP protocol\footnote{See \url{https://xdebug.org/docs/dbgp}}. This allows VDMJ to interact with a more sophisticated IDE, such as Overture. DBGP messages are exchanged over a local TCP socket, allowing the IDE to coordinate the execution of expressions within the specification, and to debug using a richer user interface. The VDMJ end of the DBGP socket coordinates the same services as the command-line does, but with requests and responses being exchanged via the socket, using DBGP messages.

So adapting VDMJ to use the LSP and DAP protocols is a matter of creating a new handler to accept socket connections from a client, and process the JSON/RPC messages defined in the respective LSP and DAP standards. Since LSP and DAP are expressed in general language terms, there is generally a natural mapping from abstract concepts in these protocols to the specific case of a VDM specification.

Creating the LSP part of the VDMJ handler was relatively simple. The biggest difference to the existing connection handlers is that LSP is an ``editing'' protocol. That is, rather than being asked to process a fixed set of unchanging specification files, LSP requires the server to accept the creation and editing of files on the fly. So whereas normally, the Parser would only be called once to process a set of fixed specification files, in the LSP handler it can be called repeatedly as edits are passed from the client. Since the VDMJ parser is relatively efficient, it is responsive enough to re-parse the affected file as edits are made. A decision was taken to only type-check the specification when the client deliberately saves the work (\ie writes changes to disk). This is the same behaviour as Overture.

Execution and debugging via the DAP protocol required the creation of a new ``DebugLink'' subclass in VDMJ. The existing command-line and DBGP protocols each extend an abstract DebugLink class, which allows the Interpreter service to interact with an arbitrary client to coordinate a debugging session. In this case, the client is the DAP client. Since the DebugLink was designed to be extended, this was relatively straightforward -- in fact the DAPDebugLink is an extension of the command-line class with the protocol aspects changed from textual read/writes to JSON message exchanges. It is about 200 lines of Java. The only complexity in this area is in the case of multi-threaded VDM++ specifications. Special care must be taken to be sure that all of the separate threads and their data are coordinated correctly, with appropriate mutex protection of the (single) communication channel to the DAP client.

In addition to parsing, type-checking and executing a specification, the LSP protocol also enables the server to offer various language services that allow the client to build a more intelligent user interface. For example, the outline of a file (its contents, in terms of the VDM definitions within and their location) can be queried; any name symbol in a file can be used to navigate to that symbol's definition (\eg moving from a function application to its definition, possibly in a different file); and name-completion services are offered, where the first few characters of a name can be typed, and the server will offer possible completions. These services do not exist in the base VDMJ, and were therefore added as part of the LSP development. They are mostly implemented via visitors (using the VDMJ visitor framework) which process the AST.

The Proof Obligation Generation and Combinatorial Testing features of VDMJ are maked available with the SLSP protocol by adding new ``slsp'' RPC methods. Internally, the server routes these new requests to the VDMJ components that are able to perform the analyses.

Proof Obligations (POs) can be generated relatively quickly (usually in a fraction of a second, even for hundreds of obligations), so the ``slsp/POG/generate'' method takes a one-shot approach, generating and returning all the POs in the specification by default, optionally allowing the UI to limit the scope to a sub-folder of specification files or a single file. The returned obligations are represented as VDM source, as a stack of contexts with a primitive obligation at the end. This allows the UI to decide how to represent the indentation of the full obligation without requiring it to understand the VDM AST.

Combinatorial Testing is a more complex problem, requiring multiple interactions between the UI and the server as new ``slsp/CT'' methods. Unlike Proof Obligations, Combinatorial Tests can expand to millions of test cases and their execution can take many hours. This in turn means that the UI must have some indication of the progress of the execution, and it must also have the ability to cleanly terminate the execution in the event that the test run is taking too long. The base LSP protocol allows for the asynchronous cancellation of an action, and this is implemented in the LSP Server by running CT in a separate thread, allowing the main thread to listen for more interactions from the UI. This complication means that a check has to be added to prevent the user from trying to launch more than one test execution at the same time (which the runtime could not easily support). The server also has to guard against changes to the specification between the expansion of the tests and their subsequent execution. Once a test run is complete, individual tests can be sent to the Interpreter for debugging. This is enabled via the standard DAP protocol, with the addition of a new ``runtrace'' launch command. So the runtime thinks that the user has started a normal interactive debugging session, but instead of executing something like ``print fac(10)'', they are executing ``runtrace A'Test 1234'', which will debug test number 1234 of the expansion of the A'Test trace.

In terms of packaging, the SLSP/DAP combination of server functionality is in its own jar, separate from (and dependent on) the standard VDMJ jar. The SLSP/DAP jar is about 174Kb. VDMJ itself is about 2.4Mb.

==> 3-Oda/sections/relatedWork.tex <==
% Not using LSP:
% Tran&19 - Migrating Overture to a different IDE
% Oda&15 - VDMPad: A Lightweight IDE for Exploratory VDM-SL Specification. 
% Thesis - Reimer&16 - An Open-source Web IDE for VDM-SL

% Using LSP:
% Rodriguez&18 - Towards a Language Server Protocol Infrastructure for Graphical Modeling
% Masci&19 - An Integrated Development Environment for the Prototype Verification System
% Hess&19 - Dafny Language Server Redesign
% Bunder19b - Towards Multi-editor Support for Domain-Specific Languages Utilizing the Language Server Protocol

% \todo[inline]{Add something about: Masci implements features outside LSP, but without using a language-agnostic protocol -> could be interesting to see if SLSP can be used there}

Support for multiple editors has become common for programming languages, and similar work is now being conducted to achieve the same for modelling and specification languages. 
Previous work has been focused on providing VDM support for specific platforms, such as Emacs \cite{Tran&19}, VDMPad \cite{Oda&15} and Overture Web IDE \cite{Reimer&16}.
For programming languages it is common to provide language support using standardised protocols to contain the language support in a language-specific server that can be used with multiple language-agnostic clients.
This tendency is also becoming apparent for other computer-based languages, such as domain-specific languages (DSL) \cite{Bunder19b}, graphical modelling \cite{Rodriguez&18} and formal specification languages such as PVS \cite{Masci&19}, Dafny \cite{Hess&19} and our work for VDM.

Tran and Kulik \cite{Tran&19} is able to migrate the Overture core from the Eclipse IDE to Emacs. 
This is carried out using as many Emacs packages as possible which allows them to provide VDM support with very few additional LoC. 
This is interesting as it provides knowledge about how few LoC is necessary, which reduces the potential gain from a generalised solution, \ie if the generalised solution requires a lot of effort you could argue that you might as well have several small dedicated solutions.

Both Oda et al. \cite{Oda&15} and Reimer and Saaby \cite{Reimer&16} presents a web IDE for VDM, based on VDMJ and Overture respectively. 
Even though both are web based they do not utilise the same language core, thus not providing the same set of language features.
Both solutions can probably benefit from unifying the efforts towards shared language support, this could be facilitated using the LSP, DAP and SLSP protocols.
Also, \gls{vscode} is build using HTML, CSS, and JavaScript which allows the IDE to be launched in a web environment, \eg Coder\footnote{See \url{https://coder.com/}.}. Thus, adding to the number of web IDEs for VDM.

% BEGIN TODO ADD IN EXTENSION
%Bünder et al. \cite{Bunder19b} create a language server for a simple DSL and implements a client for it in three different IDEs, showing that client support can be created in a short amount of time.
%Furthermore, they provide a SWOT analysis of using the LSP protocol, where they highlight the advantage of supporting multiple IDEs and find that the LSP protocol advantageously could support other types of languages.

%Rodriguez-Echeverria et al. \cite{Rodriguez&18} propose an architecture for supporting graphical modelling languages using the LSP protocol, by creating a translation scheme from nodes and edges to text and vice versa.
%This illustrates that the protocol can be used for other computer languages than programming languages, and shows that features which does not directly match the use case of the LSP protocol can still benefit from it.
% END TODO ADD IN EXTENSION

Masci and Muñoz \cite{Masci&19} provides support for PVS using the LSP protocol and VS Code. They too use the extensibility of the protocol to provide client-server support for non-LSP features, such as \gls{pog} and theorem proving.
These features are facilitated using a PVS-specific protocol.
It would be interesting to investigate if the SLSP protocol could also be used in their case, and what changes may have to be made. 
This could make way for an addition to the LSP protocol that can be used for a variety of specification languages and possibly be incorporated in the official LSP specification.





==> 3-Oda/tables/LoCCompare.tex <==
\begin{table}[htbp]
\centering
\caption{LoC measure for all IDE related files in the VS Code extension, the Emacs extension and Overture}
\label{tab:LoCCompare}
\begin{tabular}{|l|c|c|c|}
\hline
Project       & VS Code (+VDMJ)                 & Emacs                    & Overture                               \\ \hline
Lines of Code & \multicolumn{1}{r|}{1880 (+7855)} & \multicolumn{1}{r|}{349} & \multicolumn{1}{r|}{\textgreater{}63K} \\ \hline
\end{tabular}
\end{table}

==> 3-Oda/tables/LoCOverview.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htbp]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark}
\label{tab:LoCOverview}
\begin{tabular}{|l|r|r|r|r|lllrrrr}
\cline{1-5} \cline{8-12}
\multicolumn{5}{|c|}{\cellcolor[HTML]{C0C0C0}SLSP/DAP support for VDMJ}                 & \textbf{} & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{5}{c|}{\cellcolor[HTML]{C0C0C0}VS Code Extension}                                                                                                                                 \\ \cline{1-5} \cline{8-12} 
\textbf{Directory} & \textbf{Code} & \textbf{Comment} & \textbf{Blank} & \textbf{Total} &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{\textbf{Feature}} & \multicolumn{1}{r|}{\textbf{Code}} & \multicolumn{1}{r|}{\textbf{Comment}} & \multicolumn{1}{r|}{\textbf{Blank}} & \multicolumn{1}{r|}{\textbf{Total}} \\ \cline{1-5} \cline{8-12} 
dap                & 699           & 450              & 185            & 1334           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{LSP client}       & \multicolumn{1}{r|}{156}           & \multicolumn{1}{r|}{16}               & \multicolumn{1}{r|}{29}             & \multicolumn{1}{r|}{201}            \\ \cline{1-5} \cline{8-12} 
json               & 635           & 184              & 139            & 958            &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{DAP client}       & \multicolumn{1}{r|}{54}            & \multicolumn{1}{r|}{10}               & \multicolumn{1}{r|}{15}             & \multicolumn{1}{r|}{79}             \\ \cline{1-5} \cline{8-12} 
lsp                & 1653          & 625              & 337            & 2615           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{POG}              & \multicolumn{1}{r|}{460}           & \multicolumn{1}{r|}{51}               & \multicolumn{1}{r|}{96}             & \multicolumn{1}{r|}{607}            \\ \cline{1-5} \cline{8-12} 
lsp/lspx           & 169           & 44               & 30             & 243            &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{CT}               & \multicolumn{1}{r|}{732}           & \multicolumn{1}{r|}{105}              & \multicolumn{1}{r|}{165}            & \multicolumn{1}{r|}{1002}           \\ \cline{1-5} \cline{8-12} 
rpc                & 187           & 138              & 56             & 381            &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{Syntax highlight} & \multicolumn{1}{r|}{374}           & \multicolumn{1}{r|}{0}                & \multicolumn{1}{r|}{0}              & \multicolumn{1}{r|}{374}            \\ \cline{1-5} \cline{8-12} 
vdmj               & 2026          & 451              & 392            & 2869           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{SLSP protocol}    & \multicolumn{1}{r|}{104}           & \multicolumn{1}{r|}{167}              & \multicolumn{1}{r|}{27}             & \multicolumn{1}{r|}{298}            \\ \cline{1-5} \cline{8-12} 
workspace          & 2655          & 641              & 545            & 3841           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{\textbf{Sum}}     & \multicolumn{1}{r|}{\textbf{1880}} & \multicolumn{1}{r|}{\textbf{349}}     & \multicolumn{1}{r|}{\textbf{332}}   & \multicolumn{1}{r|}{\textbf{2561}}  \\ \cline{1-5} \cline{8-12} 
\textbf{Sum}       & \textbf{7855} & \textbf{2489}    & \textbf{1654}  & \textbf{11998} &           &                                &                                       &                                    &                                       &                                     &                                     \\ \cline{1-5}
\end{tabular}
\end{table}
\footnotetext{The LoC is counted using the ``VS Code Counter'' extension found at: \url{https://marketplace.visualstudio.com/items?itemName=uctakeoff.vscode-counter}}

==> 3-Oda/tables/featureCompare.tex <==
\begin{table}[htbp]
\centering
\caption{Feature comparison between the VS Code extension, Overture and Emacs. X indicates that a feature is supported. (X) indicates that the feature is only available through a command-line interface, meaning that it is not supported by a graphical user interface.}
\label{tab:featureCompare}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Features}         & \textbf{VS Code} & \textbf{Overture} & \textbf{Emacs} \\ \hline
Syntax highlighting       & X                & X                 & X              \\ \hline
Symbol prettyfication     &                  &                   & X              \\ \hline
Syntax validation         & X                & X                 & X              \\ \hline
Evaluation                & X                & X                 & (X)            \\ \hline
Debugging                 & X                & X                 & (X)            \\ \hline
POG                       & X                & X                 & (X)            \\ \hline
LaTeX report generation   &                  & X                 & (X)            \\ \hline
Combinatorial testing     & X                & X                 & (X)            \\ \hline
Code generation           &                  & X                 &                \\ \hline
Auto completion (limited) & X                & X                 & X              \\ \hline
Template expansion        &                  & X                 & X              \\ \hline
Standard library import   &                  & X                 &                \\ \hline
\end{tabular}
\end{table}

==> 4-Kulik/conclusion.tex <==
% !TEX root = ../main.tex
This paper reports on the extension of the security analysis of a sandboxing platform developed and operated as part of a project aimed at collaborative use of model based design. We created a model of the system, considering features provided within a table of roles and profiles by the implementation team. To model this feature set we have considered the mentioned actions and modeled the roles and profiles as VDM pre and post-conditions. We have then analysed several specific scenarios within the model by use of the combinatorial testing.
The analysis has in total considered 19 tests and could be carried out in about 10 seconds.

Extensions of our results should be made to allow the integration of the model checks with the implementation. The different teams involved in the security and implementation tasks closely cooperate and share access to the formal specification and the implementation, thus a potential improvement is the addition of automation to the development cycle. This work has proven valuable to the platform implementation and hence we intend to continue analyzing future updates to the platform using VDM.


==> 4-Kulik/introduction.tex <==
% !TEX root = ../main.tex
The HUBCAP project provides a collaboration platform facilitating model-based development of Cyber-Physical Systems~\cite{Macedo&21}. The platform provides resources to virtualization as a vehicle to deliver tools \cite{Badicu&21,Weiss&21} and models to its users via a typical web interface~\cite{Larsen&20c,Larsen&20d}. Tools  are understood as software necessary to develop/explore/execute a model. A tool is installed on top of an operating system, utilizing the dependencies (runtime, libraries,...) and functionality (scripts, services, connections,...) required to run it. 

The platform features a social collaboration web portal and a so called sandbox feature: \textit{an isolated temporary set of virtual machines (a customized workspace) where potential users can try out (or provide) HUBCAP assets (models and tools), using a set of tools and models without any financial charges or the need to install new software in the user's machine}. The sandbox approach brings several implementation challenges, especially in terms of security. For example, protecting the platform from malware \cite{Macedo&13}, and ensuring the protection of intellectual property of tool and model owners require standard access rights policies.  Access rights including the user roles and profiles have been implemented in the HUBCAP Sandboxing Middleware (HSM) and have been analyzed in a previous study~\cite{Kulik&20}. In this work we extend the security analysis to cover the new features of the HSM such as updates for tools located within the platform, the ability to make a tool private to restrict access to only its owner, who can share it within a Sandbox with users authorized by himself and increasing isolation of the sandbox from other parts of the platform. 

To study the security of the updated HSM we have utilized Vienna Development Method (VDM) to specify the interactions between the platform users and a formal specification of the HSM functionality. Furthermore, we specify the intra-sandbox interactions between the tools and models and represent the ability of the sandbox to act as a separate and isolated entity from the rest of the platform. VDM has been selected as a tool for analysis as it provides a formal specification system with the ability to formally analyze specific scenarios and as a formal method it has been used in asserting security in the midst of other tools~\cite{kulik2021survey}. In concrete terms, we have utilized the ISO standardized VDM-SL dialect, that has been certified by the International Standardization Organization~\cite{ISOVDM96,Plat&92b}, providing contract based modeling. The VDM modeling system uses logic, specifically use of pre-conditions, post-conditions and invariants to express properties that need to be satisfied within the model for specific scenarios. The VDM modeling system provides several tools to assist with the modeling and analysis efforts, specifically the Overture/VDM tool support~\cite{Larsen01,Larsen&10a} as well as plugins for popular text editors such as Visual Studio Code~\cite{rask&21} and Emacs~\cite{tran&19}. The VDM models have precise semantics and provide a good basis for communication of findings to the HUBCAP platform implementation team.


%One of the important aspects of security of the platform is to check whether any new functionality breaks the user access requirements that has been previously analyzed. Further the platform introduced several new concepts such as updates for tools located within the platform, possibility to fine grain access to only specific tools and models within a sandbox with a feature called \textit{private tool} and increasing isolation of the sandbox from other parts of the platform. This paper provides a reflection on the continuous security analysis of an evolving virtualized platform with significant amount of potential users accessing the platform using connections that cannot always be considered secure.


Our work is an ongoing security analysis of an evolving platform, hence we are utilizing close collaboration with the implementation team to ensure that newly implemented and planned features are analyzed for potential security issues. As the platform is evolving rapidly we are not able to obtain full coverage of security properties within the platform during the development phase, however it is our consideration that our approach would provide a significant coverage once the platform enters more stable phase in its lifecycle. 
So far the analysis has provided feedback points to the implementation team, what led to the refinement of one feature description.


The rest of the paper is organized as follows: Section~\ref{sec:arch} first describes the overall HUBCAP sandboxing middleware architecture. Section~\ref{sec:rights} contains the access rights for different actors to the sandbox environment. Afterwards, Section~\ref{sec:VDM} presents a VDM model of the security constraints for the sandbox followed by an analysis of this model in Section~\ref{sec:analyse}. Finally, Section~\ref{sec:related} provides pointers to related work while Section~\ref{sec:conclude} provides the concluding remarks.



==> 5-Fraser/background.tex <==
Anaplan is a software company that produces an eponymous, cloud-based platform for business planning.
The Anaplan platform provides a flexible model-building environment which customers use to build their own applications. These can model a simple business scenario or manage multiple, complex, planning use cases across a global enterprise, covering functions such as finance, sales, supply chain, workforce and marketing.

At the heart of Anaplan is a calculation engine that enables consistent management of OLAP (online analytical processing) cubes~\cite{codd1993providing}.
A cube (or hypercube) is a multi-dimensional array of data such that each cell represents a measure of the business.
An example cube might represent unit sales and have dimensions: products, shops, weeks, and versions (for example, actual vs forecast).
Here the value of a cell would indicate either a forecast or actual number of units sold of a given product, at a given shop, for a given week.

The dimensions of a cube are frequently hierarchical structures that model the structures inherent to the business.
For instance, shops might have parents that are cities, which in turn have parents that are countries, and similarly weeks may be grouped to align with the business's accounting periods.
These hierarchical structures can be used with an aggregation function to automatically generate additional cubes that summarize the business's data.
From our examples above, we might have a cube where each cell represents either a forecast or actual total of units sold for all products in a country, for a quarter-year period.
In Anaplan, the model builder chooses a default aggregation function, and the engine automatically calculates all possible summary cubes from the Cartesian product of hierarchical layers.

Not all of a business's data is a direct quantification of some measure, as much of it may be calculated from other data.
For instance, if we had a cube as above which represents units sold, we may have another one with the same dimensions that represents price.
Given these two cubes, we could calculate a third cube where each cell represents either a forecast or actual revenue from selling a product in a week, obtained by multiplying the values of the cells with the same coordinates from the given cubes.
Anaplan has a rich formula language, providing many inbuilt calculation functions, enabling model builders to describe all the activities of their business.
Within a single model, Anaplan immediately recalculates all necessary figures whenever the value of a cell is changed.
This makes it possible, for example, for a CEO to visualize the impact on the business's strategic plan everytime a sale is made at an integrated EPOS.

\subsection{A matter of scale}\label{subsec:a-matter-of-scale} % not a great title

A customer's Anaplan estate will typically consist of a number of connected models.
Each model will usually focus on a specific business problem, allowing detailed analysis, but will also export summarized data to be used in other models.
As mentioned previously, when any change is made within a model the impact of that change will immediately be reflected throughout the model -- akin to making a change in a spreadsheet.
Furthermore, unlike spreadsheets -- which are still commonly used for business planning -- Anaplan models will frequently have billions of cells.

To efficiently maintain the consistency of the Anaplan model, all cube data is held in memory to enable rapid retrieval and calculation.
Larger instances of models can consume more than 700GB of memory to store the cube data alone.
When the memory required to process the data, operate an API, and run the OS is added, it can take a server with 1TB of memory to operate a model.
Although such amounts of memory can be installed in your own data centres, it is at or near the limit of instances offered by cloud hosting solutions.
This is a concern as it can limit options for disaster failover.

Despite the scale of model offered by Anaplan, we are sometimes asked to provide for cubes with trillions of addressable cells.
Often this is due to practices carried over from less flexible, legacy OLAP tools, but sometimes they are due to inherent properties of the scenario being modelled and, upon closer inspection, we find that in the vast majority of these scenarios not all of these addressable cells are `valid'.
For example, an aviation company may wish to measure the time taken to fly between airports and compare it with their competitors.
According to IATA~\cite{iata}, there are approximately 9100 airports and 1100 airlines.
To track the duration of flights between any two airports by day and airline for the period of a year would require \num{3.3e13} cells.
IATA also reports~\cite{iata2} that there are less than 40 million flights made a year\footnote{In fact, many of these flights will be between the same two airports on the same day.}.
In practice, therefore, less than a thousandth of one percent of the addressable cells will ever be populated.


\subsection{An alternative calculation engine}\label{subsec:an-alternative-calculation-engine}

The Anaplan calculation engine was optimised for densely populated models.
Using large chunks of contiguous memory for cube data enables efficient calculation, aggregation, and dependency management through mechanical sympathy with the CPU caches \cite{drepper2007every}.
Although memory may not always be assigned for every addressable cell, the requirement to use contiguous memory would be inefficient for cubes like those in our example.

We decided to begin work on an alternative calculation engine that was optimised for the sparse population of a model.
Here we would only assign memory for populated cells -- enabling larger models -- and make use of sparse computation strategies to retain efficiency.
This calculation engine will be offered alongside the existing engine, enabling a user to choose appropriately for the business case they are modelling.
We would generally expect the user to be able to create the same models with either engine, and for both engines to give the same calculation results.

The calculation engine is an integral component of Anaplan, and in order to introduce another one we needed to refine the interface between the engine and the rest of the platform.
This was a task with risk, as it was critical to neither impact the functionality nor performance of the existing calculation engine.
The approach taken was to completely fork the platform, quickly make changes to the fork to determine best practice and, once established, apply production-quality changes to the mainline.
The new sparse calculation engine would then be developed in parallel and continuously integrated.
This led to having four alternative platforms available for the duration of the project: the fork and mainline platforms, each paired with either the dense or sparse engine.

\subsection{The need for formal methods}\label{subsec:the-need-for-formal-methods}

The aim of the project was to have all four platforms eventually exhibit the same behaviour.
However, there would naturally be some variation throughout the lifetime of the project.
We would be working using the agile methodology~\cite{shore2007art} and the features available in all four alternatives would vary over time and would not be equivalent at most points.

Furthermore, in some instances we wanted to alter the existing behaviour since, like most organically evolving software products, Anaplan is the culmination of design decisions made over many years.
If we were to revisit some of these decisions today, we might choose other options, as now we have more or better data that has invalidated our previous assumptions.
This is particularly true for design decisions that were influenced by the implementation method at the time or which would be made differently for a sparse paradigm.
Typically, these decisions impact performance or efficiency.

For example, consider the value of $0^0$: in Mathematics this is either left
undefined or set by convention to $0^0 = 1$, and indeed the original definition
of the $\operatorname{POWER}$ function in Anaplan follows this convention,
giving $\operatorname{POWER}(0,0) = 1$. This makes sense in a dense context,
where we can expect that the vast majority of points will have a meaningful
user-defined value. On the other hand, in a sparse context most points will not
have a user-defined value and will instead have a default value, which for
numbers is $0$. As a result, the memory consumption would be dramatically
increased if $\operatorname{POWER}(0,0)$ returned $1$, leading to performance
degradation, so for our sparse engine we chose a different convention:
$\operatorname{POWER}(0,0) = 0$.

We needed the means to not only ensure that each system exhibited the same base behaviour, but also to rigorously capture any differences between them.
We had a difficulty here as the platform has been developed using agile principles, and one of the tenets of this methodology is to prefer `working software over comprehensive documentation'~\cite{beck2001agile}.
Like most teams~\cite{wagenaar2018working}, we still possess and value documentation, but the working software is the `source of truth', and we did not have an independent means of benchmarking its correctness.

The decision was made that a specification was needed.
It was necessary that we were able to capture both the existing behaviour and any differences between the alternative platforms.
It was essential that we could do so rigorously and without ambiguity, making the use of formal methods an obvious choice.
However, we also needed the specification to fit into our agile way or working;
it would not be possible to complete the specification before starting work on the new calculation engine, and the platforms would change as the specification was written.
Furthermore, we needed to make use of the specification as soon as possible to enable quick identification and resolution of any discrepancy between the platforms' behaviour.
In summary, we needed to combine the rigour of formal methods and the flexibility of agile methods.

\subsection{Existing work}\label{subsec:related-work}

In the same way that none of the leading relational database systems satisfies Codd's twelve rules~\cite{codd1990relational}, commercial OLAP systems are inconsistent in their mathematical foundations.
Anaplan encourages the use of many small, dense, and distinct cubes that are connected through formulae to form a model.
Some of the cubes explicitly represent inputs to the model and others its outputs, such that dashboards, charts and reports are constructed automatically from those outputs.
Thus, a user does not use the typical OLAP operations, such as roll-up, drill-down, or slice and dice to {\em interact with the cube}.
Instead once a model has been constructed, the user simply makes a change and observes its immediate impact on the output artifacts.

Formalisms have been proposed for a `pure' OLAP approach~\cite{macedo2015linear,lenz2009formal}, but these have focused on the use of operations -- particularly roll-up -- within a single cube;
our specification needed to guarantee consistency across a directed graph of cubes.
Furthermore, Anaplan's connected planning methodology enables the use of multiple models -- where each typically corresponds to an area of a business -- and our specification was also required to define the asynchronous relationships between models.
These differences, and a desire to use the same methods throughout, discouraged us from pursuing the use of an existing OLAP specification.



==> 5-Fraser/introduction.tex <==
Agile methods are becoming ubiquitous in modern software engineering companies.
Meanwhile, formal methods are seen as having limited use, with the perception being that they can only provide value in niche industries, such as safety-critical systems or chip development.
In our experience, many software developers maintain a view that formal methods are incomprehensible, are tied to linear development practices, and are incompatible with agile methods.

In this paper, we seek to show that formal methods are not mutually exclusive with agile methods, but can can be used alongside them to provide additional rigour in suitable projects.
We begin by introducing Anaplan, a SaaS company delivering an enterprise planning platform using an agile development process.
Having described the fundamentals of the platform, we will outline how its calculation engine is optimized for modelling the most common business scenarios.
We will then describe a scenario that could be more efficiently handled using a different approach, how that has led to the need for an alternative calculation engine, and how formal methods could help us maintain consistency between the two engines.

We then introduce the concept of behaviour driven specification (BDS), an agile-compatible methodology that we have developed to drive specification from stakeholder requirements, and which we have used to help deliver the above calculation engine.
BDS is designed to enable specifiers to operate with agility, but we will also describe how it can be integrated into the wider agile process of a software project.

Finally, we present some metrics from our project that exemplify the impact that using BDS has had on our project, and conclude that it is feasible to successfully combine agile and formal methods in an industrial setting.


==> 5-Fraser/results.tex <==
Behaviour driven specification was not a fully-formed concept when we began, but -- like all agile processes -- has evolved as the project progressed.
We believe that the use of BDS not only has enabled us to deliver more efficiently, but has produced a more maintainable specification where behaviours are encapsulated and decoupled.
In total, we have used BDS to create more than 60,000 lines of VDM-SL, of which 26,000 lines are the 231 modules that form the specification.
There are also 115 modules of VDM-based unit tests, containing more than 3,000 tests and comprising 34,000 lines.

Our specification is split into multiple projects and we use the Gradle plugin presented in~\cite{fraser2018integrating} to manage dependencies between them.
This enables us to apply a greater degree of componentization than VDM-SL provides out-of-the-box and prevents specifiers accidentally using information that they {\em should not} know about.
For example, we have a `hierarchical data' project that has a dependency declared on an `ordered data' project.
When working in the hierarchical data project, the specifier can use modules from the ordered data project, but when working in the ordered data project the specifier cannot use modules from the hierarchy data project.
The underlying dependency mechanism is the same one Gradle uses for Java;
dependencies are acquired transitively without redeclaration and cyclic dependencies are forbidden.

Our specification is split into 54 VDM-SL projects that are all depended upon -- directly or transitively -- by a `system' project, which is published to the company's Artifactory instance and used by the VDM adapter for running the EACs.

We additionally have seven library projects which provide Java implementations for VDM modules.
For the most part, these provide speedy implementations for generic functionality that is not specific to our problem.
For instance, we have libraries for IEEE-754 floating point, ISO-8601 dates, and for standard graph algorithms.
We also used JNI to create a Rust-based library to overcome Java's limitations with Unicode characters outside the Basic Multilingual Plane.

In hindsight, we should have used libraries more heavily to provide the execution mechanisms for our functions, and focussed on solely writing VDM-SL pre and post-conditions.
As we added more and more EACs, and particularly as we generated larger scenarios, the speed of animating the specification became restrictive, and we had to make compromises in our approach;
this was particularly true when a scenario had a large memory footprint and garbage collection became a significant proportion of the runtime.

One reason that we did not completely embrace library modules earlier in the project was that we already had fully-tested VDM from a previous project, which we were not keen to throw away.
What we would like to have seen is the capability to use a library with a module where function definitions were provided with a runtime flag used to select whether to use the VDM definition or the library definition.
If that were available, we would likely use the VDM definition in local work and the library definitions in the CI environment.

At time of writing we have approximately 3,000 EACs that are run against each of the four alternative platforms whenever a commit is made to the validation repository, giving us confidence that each continually meets the defined system requirements.
Once EACs are published they are also run against each of the platform implementations when commits are made to their respective repositories.
As alluded to above, running the same set of EACs against the specification on every commit has proved to be too slow.
However, we run these in a perpetual loop on a dedicated cloud instance and get immediate feedback if and when an EAC fails.
We have found that regressions are very rare in the specification, but this process is useful for capturing unintended consequences when requirements change in a related area.
We have also tended to tighten preconditions, postconditions and invariants as the project has progressed, and this continuous validation process has enabled us to quickly spot issues that low-level VDM unit tests did not catch.

As with behaviour driven development, creating a DSL and relevant adapters is a necessary part of BDS.
Although we had five adapters to maintain, it was not as onerous as it might seem: much of the complexity in Anaplan is in the point transformations that are possible within the geometry of the cubes.
These transformations are expressed in Anaplan's formula syntax, and early on in the project we established conventions within the adapters for automatically mapping keywords into functions within the specification.
We introduced a special module -- \texttt{AnaplanFormulaFunctions} -- into our specification which served as an `interface' for these keywords.
For instance, in listing~\ref{lst:animation}, we can see that the formula keyword from listing~\ref{lst:sparse} has been converted by convention to \texttt{POWER\_SPARSE\_2}\footnote{As it has two arguments and uses the sparse arithmetic. The number of arguments is not important in this instance, but is needed as Anaplan formula syntax allows overloading, but VDM-SL does not.}.
The specifier creates a value in the \texttt{AnaplanFormulaFunctions} module that is an alias to the actual definition that they can specify in the most appropriate location.
Similarly, the VDM adapter runs a pre-build process to generate stubs for all exported parts of the specification, so that we can ensure compile-time consistency between the specification and adapter.
The four implementation adapaters were all based on the same abstract adapter and only varied where they supported different capabilities or where the code of the alternative platforms was not consistent.

One of the most important outputs of the specification process has been the identification of differences between the sparse and dense calculation engines.
Nearly 200 differences have been captured by the specification team, and it is highly unlikely that they would have been discovered by other means.
Each of these has been fully discussed and an informed, justified decision has been made.
These differences can now be fully documented {\em before} a customer encounters them, so when they do they will not only be able to see that the difference is intentional, but they will be able to view the reasoning behind it.

For the members of the specification team, BDS has had another benefit.
We have grown the size of the team from two to seven during the course of the project, with new members having varied backgrounds.
BDS enforces the breakdown of work into small, distinct chunks, which we have found to enable new members of the team to make meaningful contributions early in their tenure.
It is reasonably easy for anyone to learn to analyse a behaviour and write EACs quickly, and doing so gives new members confidence to alter the specification -- they really understand the change needed even if they do not understand the whole specification.
Similarly, it allows a more experienced specifier to move more easily to an area of the specification they have not worked with before -- they can select some simple EACs and run through how they are handled by the specification, then add some basic EACs for their new behaviour.
The EAC-driven workflow really helps comprehension of the specification, even for those who already have VDM expertise.

\section{Future work}\label{subsec:future-work}
We have begun to use the tools developed for BDS to assist with verifying our implementations.
We are constructing a verification framework that generates semi-random scenarios from the instructions available in the DSL and runs them against target systems.
These scenarios are slightly more expressive than those used for validation.
For example, it is possible to use a query to determine the valid points in a cube and then check that the value at each point in the target system satisfies the specification.

Briefly, the verification process proceeds as follows:

\begin{enumerate}
    \item Generate a scenario.
    \item Check that the {\em given} and {\em whenever} blocks satisfy the specification -- that is, that the scenario satisfies the precondition and that the command make sense.
    \item Run the scenario against the implementation in a mode that queries rather than checks.
    \item Use the results of the query to generate an equivalent scenario containing a {\em then} block, and run that scenario against the specification.
\end{enumerate}

\noindent
At the time of writing, we are continuing to develop the verification framework, and we are also scaling up its use in checking the correctness of the alternative calculation engine.
Currently, we have only preliminary results, which are not yet ready for publication.

==> 6-Bottjer/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

As of today, various models of selected IMM components, associated processes, and controllers have been developed. Nevertheless, none of the models covers all aspects of an injection moulding process. Also, models are seldom open-source or available in the public domain. 
This paper develops a high-level description of the control architecture of an injection moulding machine in VDM-RT. We selected VDM as it is traditionally used to specify the discrete part of a CPS. The developed functionality includes aspects of the process, quality and safety control.
We also set up a machine-process model based on \cite{Woll&97} and conduct a first validation of the control functionality. 

To validate the model, we generated three scenarios that were used as CSV inputs to the model. Our validation of the model shows the discrete event controller model behaves as expected in the scenarios. The model intends to provide controls to the CT model and not match its behaviour, so we decided to not use the results immediately as a measure of compliance.  Our goal is to test the VDM model using data generated from the CT model. We cross-check the results by observing the response as a plot of pressure and position/velocity and the outcome is following our expectation.  

The resulting model is a first step towards a co-simulation model that is applicable to control an injection moulding machine tool in a Digital Twin setting. Currently, we are unable to accurately point towards the effective benefits beyond the theoretical model-based design advantages. The modelling activity is in its initial stages and more research is needed to couple the model with a physical system. 
%
Next steps include enriching the models, refining the VDM model and adding testing (e.g., combinatorial tests) and at a future stage towards a Digital Twin for an IMM, we plan to interface the VDM model in a co-simulation environment.  







==> 6-Bottjer/introduction.tex <==
\section{Introduction}

%HDM
% Add safety argument
% Add the functions Step SetFilling Step Cooling and Invariant
%
Since its invention in the late 19th century, the Injection Moulding Machine (IMM) has changed the plastics manufacturing industry. At the same time, the IMM design has evolved from a purely mechanical process to a full cyber-physical system  \cite{Bibow&20} that utilise a high degree of computerisation to add smart features to the process.
The development of digital models is an essential step in the process of adding smart features to a cyber-physical system. The models may serve various purposes, e.g., models may be exercised in sync with the machine operations to detect operation anomalies, a typical Digital Twin setting or used to specify the behaviour of its components and estimate the system response by simulation. One of the first modelling tasks in a new project is to elicit the requirements and properties about the physical behaviour of the machine components and the computational processes controlling them.

In this article, we report on a new model of an idealised IMM derived from our first-hand experience obtained while working with a leading company within the sector of automated plastic manufacture.
% TODO shall we erase Lego
Our work has so far materialised in a model of a controller for an injection moulding machine based on the application of the Vienna Development Method (VDM) \cite{Fitzgerald&05}.  The model intends to serve as a specification of the IMM safety, process, and quality control requirements for a typical machine that can be found on a factory floor. Given that a subset of the VDM models are executable, it is possible to validate the requirements and understanding expressed in the specification by executing 
tests, running the controller in parallel with a model of the machine components behaviours, or generating implementations of the controller to deploy in the physical machine using co-simulation \cite{Gomes&182}. In addition, it is possible to use the executable model as a basis for discussion, expertise sharing, and use it as a test bench in an academic setting.

Our work achieved a first-principles model (i.e., a model based on the governing physics) of the discrete event controller using VDM-RT \cite{Verhoef&06b} of the IMM and validated it against scenarios obtained from a continuous time model of the IMM behaviour as described in \cite{Woll&97}. We implemented the continuous time model in MATLAB and used it to generate tests for the VDM model.   
The next validation step is to connect the VDM model with the continuous time model by use of co-simulation. In addition, it is possible to use the executable model as a basis for discussion, expertise sharing, and use it as a test bench in an academic setting.

Both the VDM model and the co-simulation model are to be made publicly available \footnote{The VDM model is available at: \url{https://www.overturetool.org/download/examples/VDM++/IMMPP}.}, so they can be used in the future by engineers that are interested in modelling and simulation of IMM as well as the application of Digital Twins in a manufacturing setting. We plan to add the VDM model to the Overture examples repository and the co-simulation in the INTO-CPS Association repository \cite{Larsen&16a}.




\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Content/Figures/ModelConnectionsDiagram.pdf}
    \caption{The connection between the discrete event (DE) model and the continuous time (CT) model. The DE models change between a number of states at events occurring in time, while in the CT models the system state variables change continuously over time.}    \label{fig:connection}
\end{figure}




The remainder of the paper is organised as follows. 
Section~\ref{sec:related} provides an overview of related work, and a general overview of the injection moulding machine in Section~\ref{sec:immp}. 
Then, Section~\ref{sec:model} contains an overview of the VDM model. 
In Section~\ref{sec:validation}, we provide an account of the continuous time model and current validation of the VDM model.
Lastly, Section~\ref{sec:conclusion}  provides a conclusion, discussion of the results, and an outline of the future work.






==> 6-Bottjer/methods.tex <==
\section{Injection Moulding Machine Model in VDM-RT}




% Introduce diagram of control logic

%%%%%%%%%%%%%%%%%%%%%%%%%%% Model Introduction %%%%%%%%%%%%%%%%%%%%%%%%%%%
This document describes the model of an injection moulding machine. The purpose of the injection moulding machine is to produce plastic parts within specifications. The injection moulding machine contains plastic granulate that is heated, injected into a given shape, and solidified to yield the final part. For obtaining high quality plastic parts, it is critical to ensure that the right amount of melted plastic is injected. 
For this, temperature, pressure and screw position are machine parameters to control during the injection process. The execution of the injection cycle needs to be carried out in a specific timely manner. 

The injection moulding system consists of: 
\begin{itemize}
    \item an motor to move the screw forward and backward
    \item heaterbands to add additional energy if the temperature in the barrel is too low
    \item a pressure sensor to determine the pressure in front of the screw
    \item a position sensor to determine the position of the screw
    \item a temperature sensor to determine the temperature 
    \item a mould that needs to be closed during injection and open to eject the solidified plastic part
    \item a software controller for safe execution of the injection cycle and quality elements
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%% Model Variables and Constants %%%%%%%%%%%%%%%%%%%%%%%%%%%
Screw Position (real), 0 to some maximum number
Heaterband <ON> | <OFF>
Mould <OPEN> | <CLOSE>
%%%%%%%%%%%%%%%%%%%%%%%%%%% Controller Requirements %%%%%%%%%%%%%%%%%%%%%%%%%%%
The controller must ensure that the injection cycle is executed in a timely manner while maintaining the correct temperature, pressure and screw position.
The controller is connected to sensors and actuators that enable the controller to: 
\begin{itemize}
    \item monitor temperature
    \item monitor pressure
    \item monitor screw position
    \item monitor the status of the mould 
    \item position the screw (which increases/decreases pressure)
    \item 
\end{itemize}

The controller has three modes: 
\begin{itemize}
    \item Initialisation Mode
    \item Production Mode 
    \item Emergency stop mode
\end{itemize}

In Initialisation Mode the controller increases the temperature, opens the mould, and moves the screw backwards.

In Production Mode the controller runs through a cyclic process: 
\begin{itemize}
    \item Filling: screw moves forward to inject the plastic and fill the mould up to 95\% (position controlled)
    \item Packing: screw moves forward to fill the remaining 5\% and achieve a specific pressure (pressure controlled) 
    \item Cooling: wait for plastic to solidify 
    \item Dosing: screw moves backward to melt material for the next filling
    \item Ejecting: mould opens, element is pushed out of the mould, mould closes
\end{itemize}

In Emergency Stop Mode the controller terminates and hands over responsibility to the physical environment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
Before beginning with the actual modelling process, it is advised to have a clear purpose for the model. Thereafter, abstraction at an appropriate level can be applied to capture relevant characteristics. For defining the purpose of the model, we describe use cases identifying all actors interacting with the system. 

% Identifying requirements for the VDM model

% Define main blocks of the system and specify which to be modelled in DT and CT

Differentiate between closed loop process control and open loop phase control

Machine components and parameter
\textbf{Temperature control of the barrel and at the nozzel}
The temperature control monitors the actual temperature in the different heating zones and sends control signal to actuators. The electrical resistance heater bands are turned on and off using semi conductor relays for a specific amount of time. Commonly the heating power of the injection machine is given in percentage e.g. 50\% heating power equal to power supply to the heating bands for half the time. 
$P_{heat} = U \cdot I = R \cdot I^{2}$
$W_{heat} = \frac{U^2}{R} \cdot t$

\textbf{Injection actuator}
To begin the injection phase the open loop phase control sents a signal to the frequency converter which in turn controls the servomotor. The frequency converter controls the motor based on the set injection speed. The pressure control behind the screw has only a monitoring function in this phase. Position is feedback from the servomotor. Pressure is feedback between the gear box and the screw.
$T = \frac{P}{\omega}$ where $\omega = \frac{2 \pi n}{60}$

\textbf{Plastification actuator}
During plastification the screw rotation is controlled by feedback of the position through a frequency converter, controlling a servo motor which is connected to the screw through a gear box. The set value given from the operator to the machine is screw rotation speed. Based on the screw rotation speed the torque of the motor is controlled. Plastification stops as soon as the shot volume is achieved.

\textbf{Pressure and force measurement}
Usually injection pressure and force are measured between the screw shaft and the actuation unit of the screw. Also, the pressure during plastification is measured in front of the screw. The process parameters that are measured include injection pressure, pack and holding pressure, and back pressure.

\subsection{DT model}
The overall purpose of this VDM(++/rt) model is to describe the (high-level) control of the injection moulding process.

% Requirements
R1: The model to be developed should describe the 6 states of the injection moulding cycle.
R2: 
\subsubsection{The Environment Class}
The \textit{Environment} class contains elements of the IMM that may be replaced by CT models. It is used to mimic the behaviour of the CT world in DE domain. External inputs to the IMM include user settings for injection job,  button press to exchange of mould, button press for initialization i.e. preheat, button press for start of injection cycle, emergency stop key, on/off switch.

The environment class defines a set of reserved names for the external inputs, and an instance variable to map the input names to a sequence of readings related to points in the approximated curve (see pg. 173, Co-sim book).

A \textit{Step} operation computes the new state of the environment in periodic intervals dt.

Further, the environment class contains a \textit{mainLoop} operation. This operation determines the system time and updates the environment model reflecting the causal relationship between the external inputs and elements of the IMM. %First, the operation reads the scenario to evaluate the external inputs to the sensors. Second, elements of the 

\subsection{Sensors and Actuators}


\subsection{Controller Class}

\textbf{Controller States}
The different states of the controller:
PowerOff
PowerOn
Initialize
Idle
Manual vs Operate
And EmergencyStop

\subsection{Safety Unit Class}
e.g. endstop protection, detect if plastic elements stuck in mould



\subsection{CT model}
To transition to a Co-model, we replace the environment class by the CT model.

The CT model for the IMM describes the motion of the screw  using a 1st order ordinary differential equation during filling phase (velocity controlled):
\begin{equation}
    \tau_1 \diff{v}{t} + v = K_1 v_f
\end{equation}
where $v_f$ describes the velocity trajectory, and $tau_1$, $K_1$ are constants. 
Using Newton's Second Law the hydraulic pressure is found: 
\begin{equation}
    \diff{v}{t} = \frac{\sum F}{M} = \frac{P_{hyd}A_{hyd} - P_{brl}A_{brl} - C_f sign(v) - B_f v}{M}
\end{equation}

Polymer flows due to the displacement of the screw and the change in  pressure in the antechamber (in front of the screw). The pressure in the antechamber $P_{noz}$ equals the barrel pressure $P_{brl}$ during fill and is found using the continuity equation: 
\begin{equation}
    \diff{P_{noz}}{V_{brl}} = \frac{K_p}{V_{brl}}(A_{brl}\diff{x}{t}-Q_1)
\end{equation}

The volume of polymer in the barrel $V_{brl}$ is equal to the initial volume $V_{brl,0}$ subtracted the volume displaced by the screw motion:
\begin{equation}
    V_{brl} = V_{brl,0} - A_{brl}x
\end{equation}

The bulk modulus $K_p$, describes the resistance of the polymer to compression and is expressed using Tait equation of state (assuming constant temperature):
\begin{equation}
    K_p = \frac{P_{noz} + B_T}{C}(1 - C \log(1+\frac{P_{noz}}{B_T}))
\end{equation}

To derive the polymer flow from the nozzle into the mould cavity the momentum equation is used assuming laminar flow and incompressible fluid in a cylindrical conduit:
\begin{equation}
    \diff{Q_1}{t} \frac{P_{noz} - P_{flowfront} - \sum \frac{F_{s,i}}{A_{c,i}}}{\rho_{avg} \sum \frac{H_{L,i}}{A_{c,i}}}
\end{equation}
where $F_S,i$ is the resistiv shear force in section i, and $A_{c,i}$ is the surface area in section i. $\rho_{avg}$ is found by evaluating Tait equation of state at $T_0$ and mean nozzle pressure $P_{noz}/2$. 

To find the resistiv shear force, Cross equation is used. 

Switch-over from velocity controlled filling to pressure controlled packing happens when the total volume of the mould equals to the injection plastic volume: 
\begin{equation}
    V_{tot} = \sum V_i
\end{equation}

\textbf{Packing}

During packing the hydraulic pressure equals: 
\begin{equation}
    tau_2 \diff{P_{hyd}}{t} + P_{hyd} = K_2 P_{hold}
\end{equation}
During packing the assumption that the polymer is incompressible does not hold true. Thus, continuity and momentum equation need to be evaluated individually for each section.

The polymer density for section i: 
\begin{equation}
    \diff{\rho_i}{t} = \frac{\rho{i-1}Q_i - \rho_i Q_{i+1}}{V_i}
\end{equation}
and the flow: 
\begin{equation}
    \diff{Q_i}{t} = (P_{i-1} - P_i - \frac{1}{2} \sum \frac{F_{s,i}}{A_{c,i}}) ( \frac{\rho_{i-1}}{2} \sum \frac{H_{L,i}}{A_ {c,i}})^{-1}
\end{equation}

\textbf{Cooling}
The melt temperature during filling is assumed to be constant.
During packing the temperature of the melt starts cooling assuming perpendicular heat loss to the mould surface and no shear heating the temperature change in section i equals: 
\begin{equation}
    \diff{T_i}{t} = - \frac{U_{o,i}A_{s,i}(T_i - T_{mold})}{\rho_i V_i C_{p,i}}
\end{equation}
with the heat transfer coefficient $U_{o,i}$
\begin{equation}
    U_{o,i} = (\frac{1}{h_c} + \frac{D_{h,i}/2}{k})^{-1}
\end{equation}

The heat capacitance $C_{p,i}$ is assumed variable: 
\begin{equation}
    C_{p,i} = 
    \begin{cases}
    c_{1,u} + c_{2,u} \bar{T} + c_{3,u} e^{-c_{4,u}\bar{T_i}^2} & \text{if $\bar{T_i} \geq 0$} \\
    c_{1,l} + c_{2,l} \bar{T} + c_{3,l} e^{-c_{4,l}\bar{T_i}^2} &\text{if $\bar{T_i} < 0$} 
    \end{cases}
\end{equation}
where $\bar{T_i} = T_i - c_5$

The fraction of solidified polymer is estimated as 
\begin{equation}
    \phi_{s,i} = \frac{\int C_{p,i} d\bar{T}}{\int C_{p,i}d\bar{T}}
\end{equation}
with the integral limits from $\bar{T_i}$ to $T_m = 10K$.

The solidification of the polymer changes the hydraulic diameter, the cross-sectional area, and the surface area in section i as: 
\begin{equation}
    D_{H,i} = D_{H0,i} \sqrt{1-\phi_{s,i}}
\end{equation}
\begin{equation}
    A_{c,i} = \frac{\pi D_{H,i}^2}{4}
\end{equation}
\begin{equation}
    A_{s,i} = \pi D_{H,i} H _{L,i}
\end{equation}

The pressure in the ith conduit equals: 
\begin{equation}
    P_i = P_{i,Tait}(1- \phi{s,i})
\end{equation}


\subsection{Co-simulation approach}

==> 6-Bottjer/model.tex <==
\section{An Injection Moulding Machine Model in VDM-RT}
\label{sec:model}

In our idealised IMM, we conceive a computer/controller receiving readings from an open/close sensor on the state of the gate, a position sensor receiving the $x$ position of the screw tip, and a pressure sensor receiving the nozzle pressure readings. The controller affects the system by issuing screw tip velocity target setpoints to the injection unit local controller, issuing commands to the belt controller on whether to accept or scrap a part, and performs PD control of an electric drive returning the screw tip to the 0-position during the Cooling phase.    

Fig. \ref{fig:UML} visualises the design of the IMM which includes (1) \texttt{Actuator}, (2) \texttt{Belt}, (3)  \texttt{Controller}, \texttt{(4) Environment}, (5)  \texttt{GateSensor}, (6) \texttt{IMM\_System}, (7)  \texttt {InjectionMachine}, (8) \texttt{MotorActuator}, (9) \texttt{PositionSensor}, 

\noindent
(10) \texttt{PressureSensor} and (11) \texttt{Timer}. All components are represented as VDM-RT files. Besides, the model receives a scenario input and returns the simulation output as CSV files. Below, we highlight various relevant aspects of the model components.

% The main purpose is ..

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Content/Figures/model-structure.pdf}
    \caption{UML class diagram of the VDM-RT model for an Injection moulding machine controller. The red dotted rectangle indicates physical components of the machine tool (sensors, actuators and environment). In addition, the VDM model includes World, System and Controller classes.}
    \label{fig:UML}
\end{figure}

\subsection{World, InjectionMachine and Environment Class}
Today, injection moulding machines integrate  complex control and software systems including closed-loop process, open-loop phase, 
safety and quality control. We developed an abstract model of the control architecture of an injection moulding machine.   
This model was developed in Overture version 3.0.0. We selected the VDM-RT dialect to implement the process/machine controller, 
quality controller and data acquisition system as a distributed control architecture. 
The \texttt{World} is the top-level entry point to the model. A scenario is input from a CSV file containing time steps, screw position, 
hydraulic pressure and the order to start production of a new plastic element. The logger operation returns a CSV file after each step of the simulation.

In our current model, the \texttt{InjectionMachine} models the continuous behaviour of the injection moulding machine. The \texttt{World} controls the simulation. Whenever time advances by calling the corresponding world functionality, the current screw position and pressure are set in the \texttt{InjectionMachine}. The Step functionality in the \texttt{InjectionMachine} sets the sensor readings for both the Position and Pressure sensor. In turn, the \texttt{Controller} can only access the sensor readings to update the current believed state of the system. This separation allows investigating problems arising from a controller being out of synchronization, i.e. sampling slower than needed. 
 
The \texttt{Environment} describes the interaction of the injection moulding machine with the surrounding environment by receiving the element's output from the injection moulding process. 

\subsection{Example of Safety Analysis}
One feature of our controller is a safety switch coupled to the gate. Our model uses an invariant to check whether the gate is closed during production. Inside the Controller class, we defined 
the StateType and LockState reflecting the state of the machine and state of the gate respectively. 

\begin{vdmpp}[style=VDM, label={lst:safety}, caption={Highlights from the Controller class}]
types
	StateType   = <Filling> | <Packing> | <Cooling> | <Ejecting> | <Idle>; 
	LockState   = <Open> | <Close>;
\end{vdmpp}
The current state of the machine operation is kept track of by updating the $ctl\_state$ variable, and the state of the gate is fed to the lock variable. Accordingly, safety is verified by invoking a function that checks at no point the door is open and the machine is not idle.
\begin{vdmpp}[style=VDM, label={lst:instancevars}, caption={Instance variables used to assert safety}]
instance variables

	ctl_state : StateType;
	lock : LockState;
    inv InterlockInvariant(lock,ctl_state)
  
functions

	InterlockInvariant : LockState * StateType -> bool
	InterlockInvariant (ls,s) == (ls = <Open>) => (s = <Idle>)
\end{vdmpp}


\subsection{Example of Process Control}
The execution of the sequential open-loop process control in injection moulding is modelled by the Step function in the \texttt{Controller}. The ctl\_state instance variable represents the current process stage. For each phase, the controller logic is unique and specified in the relevant operation - FillStep, PackStep, CoolStep and EjectStep. 


\begin{vdmpp}[style=VDM, label={lst:stages}, caption={Different IMM operation stages}]
	public Step: () ==> ()
    Step() == (
		 cases ctl_state:
		    <Idle> -> return,
		    <Filling>  -> FillStep(),
		    <Packing>  -> PackStep(),
		    <Cooling>  -> CoolStep(),
		    <Ejecting> -> EjectStep() end;);
\end{vdmpp}


The FillStep operation implements the behaviour of the controller during the filling phase. With the molten plastic in the barrel and the screw tip at position 0, the screw starts rotating to push the melt into the mould. The rotation is controlled according to the desired velocity (setpoint) of the horizontal displacement of the screw tip.  The velocity setpoints, v1, v2 and v3, were obtained from the work of \cite{Woll&97} and they are set according to positions also defined in that work for x1, x2 and x3. In Listing \ref{lst:fill}, we depict the specification of the setpoint control switching based on a reading of the screw tip position sensor, and after achieving the desired position, the machine switches to PackStep by using a variable assignment function Delta. 

\begin{vdmpp}[style=VDM, label={lst:fill}, caption={Screw velocity setpoint assignment based on current position}]
	public FillStep : () ==> () 
	FillStep() == (		
		-- Fetch sensor reading
		ctl_x := IMM_System`ps.getReading();
		-- Run control flow 
		if (ctl_x < x1)
		then (IMM_System`imm.v_t := v1)
		elseif (ctl_x < x2) 
	  then (IMM_System`imm.v_t := v2)
	  elseif (ctl_x < x3) 
	  then (IMM_System`imm.v_t := v3)
	  -- Transition to Packing
	  else Delta() )
	  pre ctl_state = <Filling>;
\end{vdmpp}


The CoolStep operation implements the behaviour of the controller during the cooling phase. With the molten plastic solidified, the screw starts rotating backwards to prepare for the next injection cycle. The screw should reach a specified position to prepare exactly the amount of plastic required to fill the mould completely. This behaviour is modelled as a PD controller using the position error to set the target velocity of the screw. 

\begin{vdmpp}[style=VDM, label={lst:cool}, caption={Return to initial state of the screw using PD control}]
	public CoolStep : () ==> ()
	CoolStep() == (
		dcl t : real := IMM_System`timer.GetTime();
		dcl dt : real := (t - last_time);
		last_time := t;
		
		ctl_x_last := ctl_x;	
		ctl_x := IMM_System`ps.getReading();
			
		e_ti_last := e_ti; 
		e_ti := 0 - ctl_x_last;
		e'_ti := (e_ti - e_ti_last)/dt;
				
		IMM_System`imm.v_t := K_p * e_ti + K_d * e'_ti;
		
		if (IMM_System`timer.GetTime()-tphase >= t_cool)
  	then Delta(); )
  	pre ctl_state = <Cooling>
	post if (ctl_state = <Ejecting>) then abs (e_ti - 0) < 0.1;
\end{vdmpp}

\subsection{Example of Quality Control}
During the filling phase, constant screw velocity and reaching the screw setpoints are key to achieving a stable process. During the packing phase, the peak injection pressure dictates quality defects of the injection moulded part. Quality control monitors relevant machine parameters and automatically differentiates between good and bad quality parts. 

% TODO substitute later
\begin{vdmpp}[style=VDM, label={lst:eject}, caption={Return to initial state of the screw using PD control}]
	public EjectStep : () ==> () 
	EjectStep() == (
		let success : bool = PartIsOK()
		in if (success) then 
			ctl_bin := <OK>
		   else 
			ctl_bin := <Scrap>;		
    pre ctl_state = <Ejecting>;
\end{vdmpp}
In VDM it is easy to define the quality control by expressing a logical formula over the historical values of the x position of the screw and the hydraulic peak value inside the interval. The Boolean variable, \verb'hyd_peak_ok', is set to false in cases where the pressure is above the threshold outside the right interval.

\begin{vdmpp}[style=VDM, label={lst:PartIsOK}, caption={Part of the quality control logic defined in the VDM specification}]
	pure PartIsOK : () ==> bool
	PartIsOK () == return (ctl_x_max >= 20.3) and hyd_peak_ok and (hyd_peak_max >= 9.1);
\end{vdmpp}

==> 7-Rose/background.tex <==
\section{Background}
\label{sec:background}


\subsection{DSE support in the INTO-CPS Toolchain}
\label{sec:into}

For a brief account of related work on DSE, we direct the reader to \cite{Fitzgerald&17a} and more recently \cite{Bogomolov&21}. In the DESTECS project on embedded systems, which was largely focussed on binary multi-models (\emph{co-models}) the need for a systematic approach to DSE was identified, using the Automated Co-model Analysis features of the DESTECS tool. A range of techniques for design parameter selection were considered, including the use of screenign experiments, fractional experiments using orthogonal matrices (Taguchi methods), space-filling searches as well as exhaustive parameter sweeps~\cite{Gamble&14}.

INTO-CPS emerged as an open toolchain permitting the co-simulation of multi-models of CPSs that conform to the Functional Mockup Interface~(FMI) standard\footnote{\url{https://fmi-standard.org/}}. The toolchain supports a workflow in which a multi-model architecture represented in a SysML profile supported by the Modelio tool which can then be used to generate the FMI specifications for the interfaces of constituent models. Co-simulation is managed through a Co-simulation Orchestration Engine~(COE) known as Maestro~\cite{Thule&193}. A web-based application can be used to launch the COE.

The purpose of DSE is to evaluate multi-models under a series of co-simulations, in order to arrive at a \emph{ranking} against an \emph{objective (or cost) function} which expresses the selection criteria that are important to the developer~\cite{Fitzgerald&17a}. One or more multi-models selected on the basis of a ranking can then be taken forward for further design. In this way, DSE can be used to reduce the range of prototypes that may have to be produced and on which expensive tests may have to be performed.

INTO-CPS supports DSE by running co-simulations on selected points in the design space. Scripts implemented in a combination of Java and Python allow the analysis to be performed from the INTO-CPS Application, and the ranking to be displayed.
Fitzgerald et al.~\cite{Fitzgerald&17a} offer a systematic approach to DSE in INTO-CPS through a specific SysML profile and demonstrate feasibility of a simple GA on a line follower robot as a first closed-loop algorithm for INTO-CPS.  In this paper, we describe a recent and more comprehensive integration of GA techniques in INTO-CPS.

\subsection{Genetic Algorithms}
\label{sec:ga}
GAs are proposed by Holland~\cite{Holland92} as an adaptive heuristic approach analogous to the biological process of natural selection~\cite{Darwin&59} whereby the selection of genes occurs through internal competition leading to unfavourable genes eventually being removed from the gene pool and convergence to an optimum with some variation~\cite{Sivanandam&08}. Fig.~\ref{fig:mainloop} shows the main loop of a typical GA that aims to select a set of optimal candidate solutions. Each iteration produces a new generation of candidate solutions. These are evaluated and a selection is made by a process that typically ensures the fitter candidates are have a higher chance of selection. In order to create the next generation, these are mated, and genetic operators such as crossover and mutation are applied. Elimination may remove infeasible solutions before a decision is made on termination. This may be based on a range of criteria such as having reached specified number of generations or when improvements between iterations are below a threshold.


\begin{figure}
\centering
\includegraphics[width=0.75\columnwidth]{figures/mainloop}
\caption{\label{fig:mainloop} Outline of a Genetic Algorithm.}
\end{figure}

In our DSE context, a solution is a candidate design represented in terms of the values of the design parameters of interest. The genetic operators that have been implemented are described in Section~\ref{sec:implement} below. 


==> 7-Rose/intro.tex <==
\section{Introduction}
\label{sec:intro}

In the model-based design of Cyber-Physical Systems~(CPSs), developers work with semantically heterogeneous collections of models (which we term \emph{multi-models}) describing computational and physical processes. Co-simulation is thus of particular interest as methods for evaluating design alternatives in order to find those that best meet combinations of requirements (e.g., for performance or cost).

In this context, a \emph{design space} is a collection of multi-models that represent alternative designs for a proposed CPS. These designs differ from one another in terms of the values of \emph{design parameters}. The process of \emph{Design Space Exploration~(DSE)} aims to identify the combinations of values for design parameters that specify designs which are optimal with respect to a defined criterion. In the DESTECS project DSE is seen as a way of managing the complex embedded systems design process~\cite{Gamble&14}. More recently, DSE has been implemented in the Integrated Toolchain for Cyber-Physical Systems~(INTO-CPS\footnote{\url{https://into-cps.org/}})~\cite{Larsen&17a2}.

Exhaustive evaluation of all designs in a design space is infeasibly costly for all but the simplest multi-models. For even moderately complex multi-models, it is necessary to hunt for optimal designs by iteratively selecting subsets of designs, evaluating these and using the results to suggest where an optimal design might lie. Genetic Algorithms~(GAs), which implement optimisation methods inspired by Darwinian principles of natural selection, may provide significant performance improvements over exhaustive methods. There are, for example, suggestions that GAs are feasible for DSE in the hardware/software codesign domain~\cite{Panerati&17}. However, an implementation of GA-based DSE has not yet been integrated in the INTO-CPS toolchain to permit the evaluation of this approach.

This paper reports an implementation and initial evaluation of GAs in DSE over multi-models in the INTO-CPS toolchain\footnote{The implementation code is available at \url{https://github.com/INTO-CPS-Association/dse_scripts}}. In order to provide this implementation, it was necessary to lay groundwork by updating the INTO-CPS DSE infrastructure, identify GAs relevant to DSE, implement such algorithms in a general setting and integrate them with the toolchain. An evaluation was undertaken, comparing a GA-based approach to the exhaustive DSE for the Robotti agricultural robot previously described by Bogomolov et al.~\cite{Bogomolov&21}.

We assume  that the reader is familiar with the principle of collaborative modelling and co-simulation based on the Functional Mockup Interface~(FMI) standard employed in INTO-CPS. Section~\ref{sec:background} provides further background on DSE and GAs in INTO-CPS. Section~\ref{sec:update} briefly describes technical updates made to INTO-CPS in order to accommodate our GA-based approach. We then are in a position to describe the GA approaches implemented in INTO-CPS~(Section~\ref{sec:implement}) and the evaluation on the Robotti data~(Section~\ref{sec:case}). We discuss the study so far and potential directions for future work in Section~\ref{sec:discussion}. 

